Measuring Linear and Non-linear Galaxy Bias Using Counts-in-Cells in the Dark Energy Survey Science Verification Data

Non-linear bias measurements require a great level of control of potential systematic effects in galaxy redshift surveys. Our goal is to demonstrate the viability of using Counts-in-Cells (CiC), a statistical measure of the galaxy distribution, as a competitive method to determine linear and higher-order galaxy bias and assess clustering systematics. We measure the galaxy bias by comparing the first four moments of the galaxy density distribution with those of the dark matter distribution. We use data from the MICE simulation to evaluate the performance of this method, and subsequently perform measurements on the public Science Verification (SV) data from the Dark Energy Survey (DES). We find that the linear bias obtained with CiC is consistent with measurements of the bias performed using galaxy-galaxy clustering, galaxy-galaxy lensing, CMB lensing, and shear+clustering measurements. Furthermore, we compute the projected (2D) non-linear bias using the expansion $\delta_{g} = \sum_{k=0}^{3} (b_{k}/k!) \delta^{k}$, finding a non-zero value for $b_2$ at the $3\sigma$ level. We also check a non-local bias model and show that the linear bias measurements are robust to the addition of new parameters. We compare our 2D results to the 3D prediction and find compatibility in the large scale regime ($>30$ Mpc $h^{-1}$)

==> authors.tex <==
\author[A.~I.~Salvador, F.~J.~S\'anchez]{
\parbox{\textwidth}{
\Large
A.~I.~Salvador$^{1}$,
F.~J.~S\'anchez$^{2,3}$,
A.~Pagul$^{4,5}$,
J.~Garc\'ia-Bellido$^{1}$,
E.~Sanchez$^{3}$,
A.~Pujol$^{6,7}$,
J.~Frieman$^{8,5}$,
E.~Gaztanaga$^{9,10}$,
A.~J.~Ross$^{11}$,
I.~Sevilla-Noarbe$^{3}$,
T.~M.~C.~Abbott$^{12}$,
S.~Allam$^{8}$,
J.~Annis$^{8}$,
S.~Avila$^{13}$,
E.~Bertin$^{14,15}$,
D.~Brooks$^{16}$,
D.~L.~Burke$^{17,18}$,
A.~Carnero~Rosell$^{19,20}$,
M.~Carrasco~Kind$^{21,22}$,
J.~Carretero$^{23}$,
F.~J.~Castander$^{9,10}$,
C.~E.~Cunha$^{17}$,
J.~De~Vicente$^{3}$,
P.~Doel$^{16}$,
A.~E.~Evrard$^{24,25}$,
P.~Fosalba$^{9,10}$,
D.~Gruen$^{17,18}$,
R.~A.~Gruendl$^{21,22}$,
J.~Gschwend$^{19,20}$,
G.~Gutierrez$^{8}$,
W.~G.~Hartley$^{16,26}$,
D.~L.~Hollowood$^{27}$,
D.~J.~James$^{28}$,
K.~Kuehn$^{29}$,
N.~Kuropatkin$^{8}$,
O.~Lahav$^{16}$,
M.~Lima$^{30,19}$,
M.~March$^{31}$,
J.~L.~Marshall$^{32}$,
F.~Menanteau$^{21,22}$,
R.~Miquel$^{33,23}$,
A.~K.~Romer$^{34}$,
A.~Roodman$^{17,18}$,
V.~Scarpine$^{8}$,
R.~Schindler$^{18}$,
M.~Smith$^{35}$,
M.~Soares-Santos$^{36}$,
F.~Sobreira$^{37,19}$,
E.~Suchyta$^{38}$,
M.~E.~C.~Swanson$^{22}$,
G.~Tarle$^{25}$,
D.~Thomas$^{13}$,
V.~Vikram$^{39}$,
A.~R.~Walker$^{12}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{2}$ Department of Physics and Astronomy, University of California, Irvine, 92602, USA\\
$^{3}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{4}$ Department of Physics and Astronomy, University of California, Riverside, 92521, USA\\
$^{5}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{6}$ DEDIP/DAP, IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur- Yvette, France\\
$^{7}$ Universit\'e Paris Diderot, AIM, Sorbonne Paris Cit\'e, CEA, CNRS, F-91191 Gif-sur-Yvette, France\\
$^{8}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{9}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08193 Barcelona, Spain\\
$^{10}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{11}$ Center for Cosmology and AstroParticle Physics, Department of Physics, The Ohio State University, 191 W Woodruff Ave,Columbus OH 43210, U.S.A.\\
$^{12}$ Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile\\
$^{13}$ Institute of Cosmology \& Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{14}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{15}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{16}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{17}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{18}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{19}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{20}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{21}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{22}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{23}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{24}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{25}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{26}$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\
$^{27}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{28}$ Harvard-Smithsonian Center for Astrophysics, Cambridge, MA 02138, USA\\
$^{29}$ Australian Astronomical Observatory, North Ryde, NSW 2113, Australia\\
$^{30}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{31}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{32}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{33}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{34}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{35}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{36}$ Brandeis University, Physics Department, 415 South Street, Waltham MA 02453\\
$^{37}$ Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil\\
$^{38}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{39}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
}
}

